On the Convergence of Tsetlin Machines for the IDENTITY- and NOT Operators

The Tsetlin Machine (TM) is a recent machine learning algorithm with several distinct properties, such as interpretability, simplicity, and hardware-friendliness. Although numerous empirical evaluations report on its performance, the mathematical analysis of its convergence is still open. In this article, we analyze the convergence of the TM with only one clause involved for classification. More specifically, we examine two basic logical operators, namely, the "IDENTITY"- and "NOT" operators. Our analysis reveals that the TM, with just one clause, can converge correctly to the intended logical operator, learning from training data over an infinite time horizon. Besides, it can capture arbitrarily rare patterns and select the most accurate one when two candidate patterns are incompatible, by configuring a granularity parameter. The analysis of the convergence of the two basic operators lays the foundation for analyzing other logical operators. These analyses altogether, from a mathematical perspective, provide new insights on why TMs have obtained state-of-the-art performance on several pattern recognition problems.

==> 1 bit case TM TPAMI revision/Tables/S.tex <==
%\begin{landscape}
\begin{table}
\centering
\caption{Conditions of $s$ for TAs to converge.}
\label{Table:S}
\begin{tabular}[]{|l|l|l|}
\hline

\textbf{Actions of $\mathrm{TA}_2$} 
& \textbf{For $\mathrm{TA}_1 \rightarrow E(x)$:} 
& \textbf{For $\mathrm{TA}_1 \rightarrow I(x)$:} 
\\
\hline

$\mathrm{TA}_2=E(\neg x)$
&
$s<s_1$
&
$s>s_2$
\\
\hline

$\mathrm{TA}_2=I(\neg x)$
&
$s<s_3$
&
$s>s_3$ NA
\\
\hline
\hline

\textbf{Actions of $\mathrm{TA}_1$} 
& \textbf{For $\mathrm{TA}_2 \rightarrow E(\neg x)$:} 
& \textbf{For $\mathrm{TA}_2 \rightarrow I(\neg x)$:} 
\\
\hline

$\mathrm{TA}_1=E(x)$
&
$s<s_4$
&
$s>s_5$
\\
\hline

$\mathrm{TA}_1=I(x)$
&
$s<s_6$
&
$s>s_6$ NA
\\
\hline



\end{tabular}
\end{table}
%\end{landscape}

==> 1 bit case TM TPAMI revision/Tables/TwoBit3.tex <==
\begin{landscape}
\begin{table}
\caption{Two-bit Case 3, where $\{T_1^{1,1}, T_1^{1,2}\} = \{I, I\}$, include both $x_1$ and $\neg x_1$.}
\label{Table:TwoBit3}
\begin{tabular}[]{|l|l|l|l|}
\hline
\multicolumn{2}{|l|}{\textbf{Two-bit Case 3: }} &\textbf{$T_1^{2,1}$, (Literal $x_2$)} & \textbf{$T_1^{2,2}$, (Literal $\neg x_2$)} \\
\hline
\hline
%row1
\multirow{4}{*}
{\begin{minipage}{0.3\textwidth}
\textbf{Scenario 1: }\\
$\{T_1^{2,1}, T_1^{2,2}\}=\{I, I\}$\\
$C_{1} = x_1 \wedge \neg x_1 \wedge x_2 \wedge \neg x_2$
\end{minipage}}
&
%row1.1
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}]  = [1,1, 1]$,
Type I, 
$C_{1}(\widehat{\bold x})  = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
\begin{tikzpicture}[node distance = .35cm, font=\Huge]
    \tikzstyle{every node}=[scale=0.35]
    
    %  NODES  
    \node[state] (A) at (1,1) {};
    \node[state] (B) at (2,1) {};
    \node[state] (C) at (3,1) {};
    \node[state] (D) at (4,1) {};
    
    % LETTERS
    \node[thick] at (0,1) {$P$};
    \node[thick] at (1.5,2) {$I$};
    \node[thick] at (3.5,2) {$E$};
    
    \draw[dotted, thick] (2.5,0.5) -- (2.5,1.5);
    
    % ARROWS
    \draw[every loop]
    (A) edge[bend left] node [scale=1.2, above=0.1 of B] {$\frac{1}{s}$} (B)
    (B) edge[bend left] node{} (C);

\end{tikzpicture}
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
\begin{tikzpicture}[node distance = .35cm, font=\Huge]
    \tikzstyle{every node}=[scale=0.35]
    
    %  NODES  
    \node[state] (A) at (1,1) {};
    \node[state] (B) at (2,1) {};
    \node[state] (C) at (3,1) {};
    \node[state] (D) at (4,1) {};
    
    % LETTERS
    \node[thick] at (0,1) {$P$};
    \node[thick] at (1.5,2) {$I$};
    \node[thick] at (3.5,2) {$E$};
    
    \draw[dotted, thick] (2.5,0.5) -- (2.5,1.5);
    
    % ARROWS
    \draw[every loop]
    (A) edge[bend left] node [scale=1.2, above=0.1 of B] {$\frac{1}{s}$} (B)
    (B) edge[bend left] node{} (C);

\end{tikzpicture}
\end{minipage}
\\
\cline{2-4}
%row1.2
&
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}]  = [1,0, 0]$,
Type II, 
$C_{1}(\widehat{\bold x})   = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
\\
\cline{2-4}
%row1.3
&
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}]  = [0,1, 0]$,
Type II, 
$C_{1}(\widehat{\bold x}) = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
\\
\cline{2-4}
%row1.4
&
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}]  = [0,0, 0]$, 
Type II, 
$C_{1}(\widehat{\bold x})   = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
\\
\hline

%row2
\multirow{4}{*}
{\begin{minipage}{0.3\textwidth}
\textbf{Scenario 2:}\\
$\{T_1^{2,1}, T_1^{2,2}\}=\{I, E\}$\\
$C_{1} = x_1 \wedge \neg x_1 \wedge x_2$
\end{minipage}}
&
%row2.1
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}] = [1,1, 1]$,
Type I, 
$C_{1}(\widehat{\bold x})  = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
\begin{tikzpicture}[node distance = .35cm, font=\Huge]
    \tikzstyle{every node}=[scale=0.35]
    
    %  NODES  
    \node[state] (A) at (1,1) {};
    \node[state] (B) at (2,1) {};
    \node[state] (C) at (3,1) {};
    \node[state] (D) at (4,1) {};
    
    % LETTERS
    \node[thick] at (0,1) {$P$};
    %\node[thick] at (1.5,2) {$I$};
    %\node[thick] at (3.5,2) {$E$};
    
    \draw[dotted, thick] (2.5,0.5) -- (2.5,1.5);
    
    % ARROWS
    \draw[every loop]
    (A) edge[bend left] node [scale=1.2, above=0.1 of B] {$\frac{1}{s}$} (B)
    (B) edge[bend left] node{} (C);

\end{tikzpicture}
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
\begin{tikzpicture}[node distance = .35cm, font=\Huge]
    \tikzstyle{every node}=[scale=0.35]
    
    %  NODES  
    \node[state] (A) at (1,1) {};
    \node[state] (B) at (2,1) {};
    \node[state] (C) at (3,1) {};
    \node[state] (D) at (4,1) {};
    
    % LETTERS
    \node[thick] at (0,1) {$R$};
    %\node[thick] at (1.5,2) {$I$};
    %\node[thick] at (3.5,2) {$E$};
    
    \draw[dotted, thick] (2.5,0.5) -- (2.5,1.5);
    
    % ARROWS
    \draw[every loop]
    (C) edge[bend left] node {} (D)
    (D) edge[loop right] node [scale=1.2, above=0.1 of B] {$\frac{1}{s}$} (D);

\end{tikzpicture}
\end{minipage}
\\
\cline{2-4}
%row2.2
&
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}]  = [1,0, 0]$,
Type II, 
$C_{1}(\widehat{\bold x})   = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
\\
\cline{2-4}
%row2.3
&
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}]  = [0,1, 0]$,
Type II, 
$C_{1}(\widehat{\bold x})  = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
\\
\cline{2-4}
%row2.4
&
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}] = [0,0, 0]$,
Type II, 
$C_{1}(\widehat{\bold x}) = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
\\
\hline

%row3
\multirow{4}{*}
{\begin{minipage}{0.3\textwidth}
\textbf{Scenario 3:}\\
$\{T_1^{2,1}, T_1^{2,2}\}=\{E, I\}$\\
$C_{1} = x_1 \wedge \neg x_1 \wedge \neg x_2$
\end{minipage}}
&
%row3.1
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}]  = [1,1, 1]$,
Type I, 
$C_{1}(\widehat{\bold x})   = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
\begin{tikzpicture}[node distance = .35cm, font=\Huge]
    \tikzstyle{every node}=[scale=0.35]
    
    %  NODES  
    \node[state] (A) at (1,1) {};
    \node[state] (B) at (2,1) {};
    \node[state] (C) at (3,1) {};
    \node[state] (D) at (4,1) {};
    
    % LETTERS
    \node[thick] at (0,1) {$R$};
   % \node[thick] at (1.5,2) {$I$};
    %\node[thick] at (3.5,2) {$E$};
    
    \draw[dotted, thick] (2.5,0.5) -- (2.5,1.5);
    
    % ARROWS
    \draw[every loop]
    (C) edge[bend left] node {} (D)
    (D) edge[loop right] node [scale=1.2, above=0.1 of B] {$\frac{1}{s}$} (D);

\end{tikzpicture}
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
\begin{tikzpicture}[node distance = .35cm, font=\Huge]
    \tikzstyle{every node}=[scale=0.35]
    
    %  NODES  
    \node[state] (A) at (1,1) {};
    \node[state] (B) at (2,1) {};
    \node[state] (C) at (3,1) {};
    \node[state] (D) at (4,1) {};
    
    % LETTERS
    \node[thick] at (0,1) {$P$};
   % \node[thick] at (1.5,2) {$I$};
    %\node[thick] at (3.5,2) {$E$};
    
    \draw[dotted, thick] (2.5,0.5) -- (2.5,1.5);
    
    % ARROWS
    \draw[every loop]
    (A) edge[bend left] node [scale=1.2, above=0.1 of B] {$\frac{1}{s}$} (B)
    (B) edge[bend left] node{} (C);

\end{tikzpicture}
\end{minipage}
\\
\cline{2-4}
%row3.2
&
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}]  = [1,0, 0]$,
Type II, 
$C_{1}(\widehat{\bold x})   = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
\\
\cline{2-4}
%row3.3
&
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}]  = [0,1, 0]$,
Type II, 
$C_{1}(\widehat{\bold x})   = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
\\
\cline{2-4}
%row3.4
&
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}]  = [0,0, 0]$,
Type II, 
$C_{1}(\widehat{\bold x})   = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
\\
\hline

%row4
\multirow{4}{*}
{\begin{minipage}{0.3\textwidth}
\textbf{Scenario 4:}\\
$\{T_1^{2,1}, T_1^{2,2}\}=\{E, E\}$\\
$C_{1} = x_1 \wedge \neg x_1$
\end{minipage}}
&
%row4.1
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}]  = [1,1, 1]$,
Type I, 
$C_{1}(\widehat{\bold x})   = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
\begin{tikzpicture}[node distance = .35cm, font=\Huge]
    \tikzstyle{every node}=[scale=0.35]
    
    %  NODES  
    \node[state] (A) at (1,1) {};
    \node[state] (B) at (2,1) {};
    \node[state] (C) at (3,1) {};
    \node[state] (D) at (4,1) {};
    
    % LETTERS
    \node[thick] at (0,1) {$R$};
   % \node[thick] at (1.5,2) {$I$};
   % \node[thick] at (3.5,2) {$E$};
    
    \draw[dotted, thick] (2.5,0.5) -- (2.5,1.5);
    
    % ARROWS
    \draw[every loop]
    (C) edge[bend left] node {} (D)
    (D) edge[loop right] node [scale=1.2, above=0.1 of B] {$\frac{1}{s}$} (D);

\end{tikzpicture}
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
\begin{tikzpicture}[node distance = .35cm, font=\Huge]
    \tikzstyle{every node}=[scale=0.35]
    
    %  NODES  
    \node[state] (A) at (1,1) {};
    \node[state] (B) at (2,1) {};
    \node[state] (C) at (3,1) {};
    \node[state] (D) at (4,1) {};
    
    % LETTERS
    \node[thick] at (0,1) {$R$};
   % \node[thick] at (1.5,2) {$I$};
   % \node[thick] at (3.5,2) {$E$};
    
    \draw[dotted, thick] (2.5,0.5) -- (2.5,1.5);
    
    % ARROWS
    \draw[every loop]
    (C) edge[bend left] node {} (D)
    (D) edge[loop right] node [scale=1.2, above=0.1 of B] {$\frac{1}{s}$} (D);

\end{tikzpicture}
\end{minipage}
\\
\cline{2-4}
%row4.2
&
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}] = [1,0, 0]$,
Type II, 
$C_{1}(\widehat{\bold x})   = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
\\
\cline{2-4}
%row4.3
&
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}]  = [0,1, 0]$,
Type II, 
$C_{1}(\widehat{\bold x})   = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
\\
\cline{2-4}
%row4.4
&
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}] = [0,0, 0]$,
Type II, 
$C_{1}(\widehat{\bold x})  = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
\\
\hline


\end{tabular}
\end{table}
\end{landscape}

==> 1 bit case TM TPAMI revision/Tables/absorbingstates.tex <==
%\begin{landscape}
\begin{table*}
\centering
\caption{Three convergence possibilities of the TM.}
\label{table:absorbingstates}
\begin{tabular}[]{|l|l|l|l|}
\hline
$(\mathrm{TA}_1,\mathrm{TA}_2)$& $s$ in general case & $s$ when $c=0.5$ & $a,b$\\
\hline
\hline

$(\mathrm{TA}_1,\mathrm{TA}_2)\rightarrow (E(x), E(\neg x))$ 
& $1<s<\min(s_1,s_4)$ 
& $1<s<\min(\frac{a+b}{a+1-b},\frac{a+b}{b+1-a})$
& $a>0.5, b>0.5$
\\
\hline

$(\mathrm{TA}_1,\mathrm{TA}_2)\rightarrow (I(x), E(\neg x))$ 
& $s_2<s<s_6$ 
& $\frac{a+b}{a}<s<\frac{a+b}{1-a}$
& $a>0.5$
\\
\hline

$(\mathrm{TA}_1,\mathrm{TA}_2)\rightarrow (E(x), I(\neg x))$ 
& $s_5<s<s_3$ 
& $\frac{a+b}{b}<s<\frac{a+b}{1-b}$
& $b>0.5$
\\
\hline

\end{tabular}
\end{table*}
%\end{landscape}


%%\begin{landscape}
%\begin{table*}
%\centering
%%\resizebox{\columnwidth}{!}{
%\caption{Three absorbing states of the TM}
%\label{table:absorbingstates}
%\begin{tabular}[]{|l|l|l|l|}
%\hline
%$(\mathrm{TA}_1,\mathrm{TA}_2)\rightarrow $& $s$ in general & $s$ when $c=0.5$ & $a,b$\\
%\hline
%\hline
%
%$(E(x), E(\neg x))$ 
%& $(1,\min(s_1,s4))$ 
%& $(1,\min(\frac{a+b}{a+1-b},\frac{a+b}{b+1-a}))$
%& $a,b>0.5$
%\\
%\hline
%
%$(I(x), E(\neg x))$ 
%& $(s_2,s_6)$ 
%& $(\frac{a+b}{a},\frac{a+b}{1-a})$
%& $a>0.5$
%\\
%\hline
%
%$(E(x), I(\neg x))$ 
%& $(s_5,s_3)$ 
%& $(\frac{a+b}{b},\frac{a+b}{1-b})$
%& $b>0.5$
%\\
%\hline
%
%\end{tabular}
%%}
%\end{table*}
%%\end{landscape}

==> Tables/TwoBit3.tex <==
\begin{landscape}
\begin{table}
\caption{Two-bit Case 3, where $\{T_1^{1,1}, T_1^{1,2}\} = \{I, I\}$, include both $x_1$ and $\neg x_1$.}
\label{Table:TwoBit3}
\begin{tabular}[]{|l|l|l|l|}
\hline
\multicolumn{2}{|l|}{\textbf{Two-bit Case 3: }} &\textbf{$T_1^{2,1}$, (Literal $x_2$)} & \textbf{$T_1^{2,2}$, (Literal $\neg x_2$)} \\
\hline
\hline
%row1
\multirow{4}{*}
{\begin{minipage}{0.3\textwidth}
\textbf{Scenario 1: }\\
$\{T_1^{2,1}, T_1^{2,2}\}=\{I, I\}$\\
$C_{1} = x_1 \wedge \neg x_1 \wedge x_2 \wedge \neg x_2$
\end{minipage}}
&
%row1.1
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}]  = [1,1, 1]$,
Type I, 
$C_{1}(\widehat{\bold x})  = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
\begin{tikzpicture}[node distance = .35cm, font=\Huge]
    \tikzstyle{every node}=[scale=0.35]
    
    %  NODES  
    \node[state] (A) at (1,1) {};
    \node[state] (B) at (2,1) {};
    \node[state] (C) at (3,1) {};
    \node[state] (D) at (4,1) {};
    
    % LETTERS
    \node[thick] at (0,1) {$P$};
    \node[thick] at (1.5,2) {$I$};
    \node[thick] at (3.5,2) {$E$};
    
    \draw[dotted, thick] (2.5,0.5) -- (2.5,1.5);
    
    % ARROWS
    \draw[every loop]
    (A) edge[bend left] node [scale=1.2, above=0.1 of B] {$\frac{1}{s}$} (B)
    (B) edge[bend left] node{} (C);

\end{tikzpicture}
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
\begin{tikzpicture}[node distance = .35cm, font=\Huge]
    \tikzstyle{every node}=[scale=0.35]
    
    %  NODES  
    \node[state] (A) at (1,1) {};
    \node[state] (B) at (2,1) {};
    \node[state] (C) at (3,1) {};
    \node[state] (D) at (4,1) {};
    
    % LETTERS
    \node[thick] at (0,1) {$P$};
    \node[thick] at (1.5,2) {$I$};
    \node[thick] at (3.5,2) {$E$};
    
    \draw[dotted, thick] (2.5,0.5) -- (2.5,1.5);
    
    % ARROWS
    \draw[every loop]
    (A) edge[bend left] node [scale=1.2, above=0.1 of B] {$\frac{1}{s}$} (B)
    (B) edge[bend left] node{} (C);

\end{tikzpicture}
\end{minipage}
\\
\cline{2-4}
%row1.2
&
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}]  = [1,0, 0]$,
Type II, 
$C_{1}(\widehat{\bold x})   = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
\\
\cline{2-4}
%row1.3
&
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}]  = [0,1, 0]$,
Type II, 
$C_{1}(\widehat{\bold x}) = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
\\
\cline{2-4}
%row1.4
&
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}]  = [0,0, 0]$, 
Type II, 
$C_{1}(\widehat{\bold x})   = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
\\
\hline

%row2
\multirow{4}{*}
{\begin{minipage}{0.3\textwidth}
\textbf{Scenario 2:}\\
$\{T_1^{2,1}, T_1^{2,2}\}=\{I, E\}$\\
$C_{1} = x_1 \wedge \neg x_1 \wedge x_2$
\end{minipage}}
&
%row2.1
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}] = [1,1, 1]$,
Type I, 
$C_{1}(\widehat{\bold x})  = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
\begin{tikzpicture}[node distance = .35cm, font=\Huge]
    \tikzstyle{every node}=[scale=0.35]
    
    %  NODES  
    \node[state] (A) at (1,1) {};
    \node[state] (B) at (2,1) {};
    \node[state] (C) at (3,1) {};
    \node[state] (D) at (4,1) {};
    
    % LETTERS
    \node[thick] at (0,1) {$P$};
    %\node[thick] at (1.5,2) {$I$};
    %\node[thick] at (3.5,2) {$E$};
    
    \draw[dotted, thick] (2.5,0.5) -- (2.5,1.5);
    
    % ARROWS
    \draw[every loop]
    (A) edge[bend left] node [scale=1.2, above=0.1 of B] {$\frac{1}{s}$} (B)
    (B) edge[bend left] node{} (C);

\end{tikzpicture}
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
\begin{tikzpicture}[node distance = .35cm, font=\Huge]
    \tikzstyle{every node}=[scale=0.35]
    
    %  NODES  
    \node[state] (A) at (1,1) {};
    \node[state] (B) at (2,1) {};
    \node[state] (C) at (3,1) {};
    \node[state] (D) at (4,1) {};
    
    % LETTERS
    \node[thick] at (0,1) {$R$};
    %\node[thick] at (1.5,2) {$I$};
    %\node[thick] at (3.5,2) {$E$};
    
    \draw[dotted, thick] (2.5,0.5) -- (2.5,1.5);
    
    % ARROWS
    \draw[every loop]
    (C) edge[bend left] node {} (D)
    (D) edge[loop right] node [scale=1.2, above=0.1 of B] {$\frac{1}{s}$} (D);

\end{tikzpicture}
\end{minipage}
\\
\cline{2-4}
%row2.2
&
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}]  = [1,0, 0]$,
Type II, 
$C_{1}(\widehat{\bold x})   = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
\\
\cline{2-4}
%row2.3
&
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}]  = [0,1, 0]$,
Type II, 
$C_{1}(\widehat{\bold x})  = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
\\
\cline{2-4}
%row2.4
&
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}] = [0,0, 0]$,
Type II, 
$C_{1}(\widehat{\bold x}) = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
\\
\hline

%row3
\multirow{4}{*}
{\begin{minipage}{0.3\textwidth}
\textbf{Scenario 3:}\\
$\{T_1^{2,1}, T_1^{2,2}\}=\{E, I\}$\\
$C_{1} = x_1 \wedge \neg x_1 \wedge \neg x_2$
\end{minipage}}
&
%row3.1
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}]  = [1,1, 1]$,
Type I, 
$C_{1}(\widehat{\bold x})   = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
\begin{tikzpicture}[node distance = .35cm, font=\Huge]
    \tikzstyle{every node}=[scale=0.35]
    
    %  NODES  
    \node[state] (A) at (1,1) {};
    \node[state] (B) at (2,1) {};
    \node[state] (C) at (3,1) {};
    \node[state] (D) at (4,1) {};
    
    % LETTERS
    \node[thick] at (0,1) {$R$};
   % \node[thick] at (1.5,2) {$I$};
    %\node[thick] at (3.5,2) {$E$};
    
    \draw[dotted, thick] (2.5,0.5) -- (2.5,1.5);
    
    % ARROWS
    \draw[every loop]
    (C) edge[bend left] node {} (D)
    (D) edge[loop right] node [scale=1.2, above=0.1 of B] {$\frac{1}{s}$} (D);

\end{tikzpicture}
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
\begin{tikzpicture}[node distance = .35cm, font=\Huge]
    \tikzstyle{every node}=[scale=0.35]
    
    %  NODES  
    \node[state] (A) at (1,1) {};
    \node[state] (B) at (2,1) {};
    \node[state] (C) at (3,1) {};
    \node[state] (D) at (4,1) {};
    
    % LETTERS
    \node[thick] at (0,1) {$P$};
   % \node[thick] at (1.5,2) {$I$};
    %\node[thick] at (3.5,2) {$E$};
    
    \draw[dotted, thick] (2.5,0.5) -- (2.5,1.5);
    
    % ARROWS
    \draw[every loop]
    (A) edge[bend left] node [scale=1.2, above=0.1 of B] {$\frac{1}{s}$} (B)
    (B) edge[bend left] node{} (C);

\end{tikzpicture}
\end{minipage}
\\
\cline{2-4}
%row3.2
&
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}]  = [1,0, 0]$,
Type II, 
$C_{1}(\widehat{\bold x})   = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
\\
\cline{2-4}
%row3.3
&
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}]  = [0,1, 0]$,
Type II, 
$C_{1}(\widehat{\bold x})   = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
\\
\cline{2-4}
%row3.4
&
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}]  = [0,0, 0]$,
Type II, 
$C_{1}(\widehat{\bold x})   = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
\\
\hline

%row4
\multirow{4}{*}
{\begin{minipage}{0.3\textwidth}
\textbf{Scenario 4:}\\
$\{T_1^{2,1}, T_1^{2,2}\}=\{E, E\}$\\
$C_{1} = x_1 \wedge \neg x_1$
\end{minipage}}
&
%row4.1
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}]  = [1,1, 1]$,
Type I, 
$C_{1}(\widehat{\bold x})   = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
\begin{tikzpicture}[node distance = .35cm, font=\Huge]
    \tikzstyle{every node}=[scale=0.35]
    
    %  NODES  
    \node[state] (A) at (1,1) {};
    \node[state] (B) at (2,1) {};
    \node[state] (C) at (3,1) {};
    \node[state] (D) at (4,1) {};
    
    % LETTERS
    \node[thick] at (0,1) {$R$};
   % \node[thick] at (1.5,2) {$I$};
   % \node[thick] at (3.5,2) {$E$};
    
    \draw[dotted, thick] (2.5,0.5) -- (2.5,1.5);
    
    % ARROWS
    \draw[every loop]
    (C) edge[bend left] node {} (D)
    (D) edge[loop right] node [scale=1.2, above=0.1 of B] {$\frac{1}{s}$} (D);

\end{tikzpicture}
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
\begin{tikzpicture}[node distance = .35cm, font=\Huge]
    \tikzstyle{every node}=[scale=0.35]
    
    %  NODES  
    \node[state] (A) at (1,1) {};
    \node[state] (B) at (2,1) {};
    \node[state] (C) at (3,1) {};
    \node[state] (D) at (4,1) {};
    
    % LETTERS
    \node[thick] at (0,1) {$R$};
   % \node[thick] at (1.5,2) {$I$};
   % \node[thick] at (3.5,2) {$E$};
    
    \draw[dotted, thick] (2.5,0.5) -- (2.5,1.5);
    
    % ARROWS
    \draw[every loop]
    (C) edge[bend left] node {} (D)
    (D) edge[loop right] node [scale=1.2, above=0.1 of B] {$\frac{1}{s}$} (D);

\end{tikzpicture}
\end{minipage}
\\
\cline{2-4}
%row4.2
&
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}] = [1,0, 0]$,
Type II, 
$C_{1}(\widehat{\bold x})   = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
\\
\cline{2-4}
%row4.3
&
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}]  = [0,1, 0]$,
Type II, 
$C_{1}(\widehat{\bold x})   = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
\\
\cline{2-4}
%row4.4
&
\begin{minipage}{0.4\textwidth}
$[\widehat{\bold x}, \widehat{y}] = [0,0, 0]$,
Type II, 
$C_{1}(\widehat{\bold x})  = 0$
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
&
\begin{minipage}{0.35\textwidth}
No change.
\end{minipage}
\\
\hline


\end{tabular}
\end{table}
\end{landscape}
